Assessing Transferability from Simulation to Reality for Reinforcement Learning

Learning robot control policies from physics simulations is of great interest to the robotics community as it may render the learning process faster, cheaper, and safer by alleviating the need for expensive real-world experiments. However, the direct transfer of learned behavior from simulation to reality is a major challenge. Optimizing a policy on a slightly faulty simulator can easily lead to the maximization of the `Simulation Optimization Bias` (SOB). In this case, the optimizer exploits modeling errors of the simulator such that the resulting behavior can potentially damage the robot. We tackle this challenge by applying domain randomization, i.e., randomizing the parameters of the physics simulations during learning. We propose an algorithm called Simulation-based Policy Optimization with Transferability Assessment (SPOTA) which uses an estimator of the SOB to formulate a stopping criterion for training. The introduced estimator quantifies the over-fitting to the set of domains experienced while training. Our experimental results on two different second order nonlinear systems show that the new simulation-based policy search algorithm is able to learn a control policy exclusively from a randomized simulator, which can be applied directly to real systems without any additional training.

==> plots/QBB_QQ_UCBOG_decrease.tex <==
\begin{figure*}[t!]
	\centering
	\begin{subfigure}[t]{0.495\textwidth}
		\centering
		\includegraphics[height=4.7cm,keepaspectratio]{plots/}%[height=X.XXcm,keepaspectratio] or [width=\columnwidth]
		\vspace*{-0.5ex} \caption{\vspace*{-0.7ex} Ball-Balancer}
		\label{fig_UCBOG_decrease_QBB}
	\end{subfigure}%
	\hfill
	\begin{subfigure}[t]{0.495\textwidth}
		\centering
		\includegraphics[height=4.7cm,keepaspectratio]{plots/}%[height=X.XXcm,keepaspectratio] or [width=\columnwidth]
		\vspace*{-0.5ex} \caption{\vspace*{-0.7ex} Qube}
		\label{fig_UCBOG_decrease_QQ}
	\end{subfigure}%
	\caption{%
		\acf{UCBOG} and number of candidate solution domain over the iteration count of \ac{SPOTA}. Every iteration, the number and domains and hence the sample size is increased. The shaded area visualize $\pm 1$ standard deviation across 17 training runs on the simulated Ball-Balancer.}
	\label{fig_UCBOG_decrease}
\end{figure*}


==> plots/QBB_QQ_real_eval.tex <==
\begin{figure*}[t!]
	\centering
	\begin{subfigure}[t]{0.495\textwidth}
		\centering
		\includegraphics[height=4.7cm,keepaspectratio]{plots/QBB_real_returns_boxplot.pdf}%[height=X.XXcm,keepaspectratio] or [width=\columnwidth]
		\vspace*{-0.5ex} \caption{\vspace*{-0.7ex} Ball-Balancer}
		\label{fig_real_eval_QBB}
	\end{subfigure}%
\hfill
	\begin{subfigure}[t]{0.495\textwidth}
		\centering
	        \includegraphics[height=4.7cm,keepaspectratio]{plots/QBB_real_returns_boxplot.pdf}%[height=X.XXcm,keepaspectratio] or [width=\columnwidth]
		\vspace*{-0.5ex} \caption{\vspace*{-0.7ex} Qube}
		\label{fig_real_eval_QCP}
	\end{subfigure}%
	\caption{%
		Evaluation of the learned control policies on the real Ball-Balancer (a) and the real Qube (b).
		The results were obtained from 40 rollouts per policy on the Ball-Balancer (5 repetitions for 8 different initial ball positions) as well as 10 rollouts per policy on the Qube (1 initial state).
		The dashed lines approximately mark the threshold where the tasks are solved, \ie, the ball is centered in the middle (a), or the pendulum is stabilized upright (b).
		%The mean is displayed as a purple diamond.
	}
	\label{fig_real_eval}
\end{figure*}


==> plots/QBB_QQ_sim_eval_dp_range.tex <==
\begin{figure*}[h]
	\centering
	\begin{subfigure}[t]{0.495\textwidth}
		\centering
		\includegraphics[height=5.2cm,keepaspectratio]{plots/m_ball_mean_std.pdf}%[height=X.XXcm,keepaspectratio] or [width=\columnwidth]
		\vspace*{-0.5ex} \caption{\vspace*{-0.7ex} Ball-Balancer -- varying ball mass}
		\label{fig_QBB_sim_eval_dp_range_m_ball}
	\end{subfigure}%
\hfill
	\begin{subfigure}[t]{0.495\textwidth}
		\centering
	        \includegraphics[height=5.2cm,keepaspectratio]{plots/c_frict_mean_std.pdf}%[height=.XXXcm,keepaspectratio] or [width=\columnwidth]
		\vspace*{-0.5ex} \caption{\vspace*{-0.7ex} Ball-Balancer -- varying ball viscous friction coeff.}
		\label{fig_QBB_sim_eval_dp_range_c_frict}
	\end{subfigure}%
\\[1em]
	\begin{subfigure}[t]{0.495\textwidth}
		\centering
		\includegraphics[height=5.2cm,keepaspectratio]{plots/m_ball_mean_std.pdf}%[height=X.XXcm,keepaspectratio] or [width=\columnwidth]
		\vspace*{-0.5ex} \caption{\vspace*{-0.7ex} Qube -- varying ball mass}
		\label{fig_QCP_sim_eval_dp_range_m_ball}
	\end{subfigure}%
\hfill
	\begin{subfigure}[t]{0.495\textwidth}
		\centering
		\includegraphics[height=5.2cm,keepaspectratio]{plots/c_frict_mean_std.pdf}%[height=.XXXcm,keepaspectratio] or [width=\columnwidth]
		\vspace*{-0.5ex} \caption{\vspace*{-0.7ex} Qube -- varying ball viscous friction coeff.}
		\label{fig_QCP_sim_eval_dp_range_c_frict}
	\end{subfigure}%
%
	\caption{%
		Evaluation of the learned control policies on the simulated Ball-Balancer (top row) as well as the simulated Qube (bottom row), varying the ball mass $m_b$ (a), the viscous friction coefficient (b), the ?? (c), and the ?? (d).
		Every domain parameter configuration has been evaluated on 360 rollouts with different initial states, synchronized across all policies.
		The dashed lines mark the nominal parameter values. The solid lines represent the means, and shaded areas show $\pm 1$ standard deviation
	}
	\label{fig_QBB_QQ_sim_eval_dp_range}
\end{figure*}


==> tables/domain_parameters_QQ.tex <==
\rowcolors{2}{gray!25}{white}
\begin{tabular}{lll}
	\rowcolor{gray!50}
	\textbf{Parameter}           & \textbf{Distribution}                           & \textbf{Unit}\\
	gravity constant             & $\distrnormal{g}{\num{9.81},\num{1.962}}$       & $[\si{\meter\per\second\squared}]$\\
	rotary pole mass             & $\distrnormal{m_r}{\num{0.095},\num{9.5e-3}}$   & $[\si{kg}]$\\
	pendulum pole mass           & $\distrnormal{m_p}{\num{0.024},\num{2.4e-3}}$   & $[\si{kg}]$\\
	rotary pole length           & $\distrnormal{l_r}{\num{0.085},\num{8.8e-3}}$   & $[\si{m}]$\\
	pendulum pole length         & $\distrnormal{l_p}{\num{0.129},\num{1.29e-2}}$  & $[\si{m}]$\\
	motor torque constant        & $\distrnormal{k_m}{\num{0.042},\num{4.2e-3}}$   & $[\si{\newton\meter\per\ampere}]$\\
	motor armature resistance    & $\distrnormal{R_m}{\num{8.4},\num{0.84}}$       & $[\si{\ohm}]$\\
	rotary pole viscous friction coeff.   & $\distruniform{d_r}{\num{5.0e-6},\num{5.0e-7}}$ & $$[\si{\newton\meter\second\per\radian}]$$\\
	pendulum pole viscous friction coeff. & $\distruniform{d_p}{\num{1.0e-6},\num{1.0e-7}}$ & $$[\si{\newton\meter\second\per\radian}]$$\\
	action delay                          & $\distruniform{\Delta t_a}{0,10}$               & $[\mathrm{steps}]$\\
	\hline\hline
	rotary pole inertia about \acs{CoM}   & $J_r = 1 / 12 m_r l_r^2$                        & $[\si{\kilogram\meter\squared}]$\\
	pendulum pole inertia about \acs{CoM} & $J_p = 1 / 12 m_p l_p^2$                        & $[\si{\kilogram\meter\squared}]$\\
\end{tabular}


==> tables/experiments_results.tex <==
\rowcolors{2}{gray!25}{white}
\begin{tabular}{lcccc}
	\rowcolor{gray!50}
	\textbf{Environment}        & \textbf{\acs{SPOTA}} & \textbf{\acs{EPOpt}} & \textbf{\acs{PPO}} & \textbf{\acs{PD}} \\
	Simulated Ball Balancer & $3 \pm 1$   & $3 \pm 1$   & $3 \pm 1$ & $3 \pm 1$ \\
	Real Ball balancer      & $3 \pm 1$   & $3 \pm 1$   & $3 \pm 1$ & $3 \pm 1$ \\
	Simulated Cart-Pole     & $3 \pm 1$   & $3 \pm 1$   & $3 \pm 1$ & $3 \pm 1$ \\
	Real Cart-Pole          & $3 \pm 1$   & $3 \pm 1$   & $3 \pm 1$ & $3 \pm 1$ \\
\end{tabular}

